Irreducible Canonical Representations in Positive Characteristic

For $X$ a curve over a field of positive characteristic, we investigate when the canonical representation of $\text{Aut}(X)$ on $H^0(X, \Omega_X)$ is irreducible. Any curve with an irreducible canonical representation must either be superspecial or ordinary. Having a small automorphism group is an obstruction to having irreducible canonical representation; with this motivation, the bulk of the paper is spent bounding the size of automorphism groups of superspecial and ordinary curves. After proving that all automorphisms of an $\mathbb{F}_{q^2}$-maximal curve are defined over $\mathbb{F}_{q^2}$, we find all superspecial curves with $g > 82$ having an irreducible representation. In the ordinary case, we provide a bound on the size of the automorphism group of an ordinary curve that improves on a result of Nakajima.

==> end.tex <==
\section{Curves with Irreducible Canonical Representation}

%Maybe add some concluding material here, depending on where we get to; should we re-iterate the remark about this being solved otherwise?
